High-Quality Iterative Logic Compiler for In-Memory SIMD Computation with Tight Coupling of Synthesis and Scheduling

In-memory computing (IMC) with single instruction multiple data (SIMD) setup enables memory to perform operations on the stored data in parallel to achieve high throughput and energy saving. To instruct a SIMD IMC hardware to compute a function, a logic compiler is needed that involves two steps: logic synthesis and scheduling. Logic synthesis transforms the function into a netlist of supported operations. Scheduling determines the execution sequence and memory location of the operations and outputs the instruction sequence given to the hardware. In this work, we propose an iterative logic compiler with tight coupling of synthesis and scheduling to find high-quality instruction sequences. It is based on improving the critical sub-netlist identified by our algorithm and performing problem-specific resubstitution. The experimental results show that our compiler can obtain better instruction sequences with energy-delay products reduced by 18.0% on average compared to the best state-of-the-art method.

==> 2_background.tex <==
\section{Background}\label{sec:background}
In this section, we present the background of SIMD IMC compiler, and the resubstitution in traditional logic synthesis.

\subsection{Compiler of SIMD IMC}\label{sec:back_comp}
\begin{figure}[!htbp]
\centering
\includegraphics[scale=0.71]{compiler.jpg}
\caption{(a) The flow of a SIMD IMC compiler; (b) a netlist example; (c) an example of scheduling result.}
\label{fig:compiler}
\end{figure}
To efficiently use a SIMD IMC hardware, a compiler is needed to convert the target function into the instruction sequence given to the hardware to compute it.
A basic compiler consists of two steps as shown in Fig.~\ref{fig:compiler}(a): logic synthesis and scheduling.

Logic synthesis takes the function as input and outputs a netlist of the primitive operations supported by the hardware.
In this work, we use the architecture proposed in~\cite{XMG-GPPIC} as our target architecture.
It supports inversion and 3-input XOR and MAJ operations, where the inversion is achieved by directly reading the negated output of a memory cell.
Hence, the corresponding netlist is an XMG as shown in Fig.~\ref{fig:compiler}(b).
Each node in the netlist corresponds to one supported operation, \textit{i.e.}, either XOR or MAJ, and we use the terms operation and node interchangeably.
A directed edge from node $i$ to node $j$ indicates that the output of node $i$ is an input of node $j$.
If the edge is dashed, the output of node $i$ is complemented when serving as an input of node $j$.
We call node $i$ a \emph{fan-in} of node $j$ and node $j$ a \emph{fan-out} of node $i$.
The blue variables are the \emph{primary inputs (PIs)} of the function, while the operations connected to the green variables are the \emph{primary outputs (POs)} of the function.
The PIs are initially stored in memory. Typically, they cannot be deleted during the process, since they may still be needed in the future.
The results of POs must be in memory when the computation ends, and thus also cannot be deleted once computed.
The results of other operations can be deleted from the memory once they are no longer needed to save memory space.
Here, by deleting an operation result from memory, we mean that the row containing the result can be overwritten and hence, becomes available for future operations.
Note that some operations in the figure only have two fan-ins, because we omit the constant 0 for simplicity.
Since it takes time and energy to perform each operation in the netlist in serial, in general, we want to minimize the size of the netlist to obtain a design with good performance.

The scheduler determines the execution sequence of the operations and the memory rows to store their results, and then outputs the instruction sequence given to the hardware.
Fig.~\ref{fig:compiler}(c) shows an example of a scheduling result of the netlist in Fig.~\ref{fig:compiler}(b).
The execution sequence is $N_1, N_2, N_4, N_3, N_5$, and the corresponding instruction to execute each operation is listed to the right of `:', forming the instruction sequence given to the hardware.
In SIMD IMC, the instructions are given to the rows of the hardware, and the cells in a row are processed bitwise.
When we want to compute function $f$ with multiple input patterns, we put each input pattern in the cells of column $i$, and all the operations of function $f$ with that input pattern are performed in that column.
In this way, although the operations of the function must be performed in serial, the same function $f$ with these input patterns can be computed in parallel in the $c$ columns.
For example, at clock three, the instruction given to the hardware is $R_{10}\leftarrow \textit{MAJ}(R_{10},!R_{11},R_8)$ to perform operation $N_4$, meaning that we perform an MAJ operation for each input pattern at the same time on row 10 containing the result of operation $N_1$, the complemented row 11 containing the result of operation $N_2$, and row 8 containing the PI $x_8$, and store the result at row 10.
Note that the hardware~\cite{XMG-GPPIC} supports the result of an operation to overwrite one of the rows occupied by its fan-ins.
Any instruction sequence can be used to compute the function if: 1) at the clock cycle when each operation is scheduled, \textit{i.e.}, executed, the fan-ins of the operation are stored in the memory; 2) the POs are stored in memory at the end of the process.
By performing the operations one by one, we can ideally compute the function with an arbitrarily large netlist in the memory arrays.

However, an operation can only be applied to the rows in the same memory array, and the number of rows in an array is constrained by technology limit~\cite{NVSIM}.
When the rows containing the fan-ins of an operation are from different arrays, we need to execute extra costly cross-array data copying instructions before executing the operation. This may diminish the advantage of IMC~\cite{XMG-GPPIC,SIMPLER,CHAL}.
Hence, the common target of scheduler is to minimize the MF~\cite{MIG,XMG-GPPIC,SIMPLER,STAR,LOGIC,PREV}, \textit{i.e.}, the number of rows required to store the operation results.
For example, for the instruction sequence in Fig.~\ref{fig:compiler}(c), the MF is two, since two rows, \textit{i.e.}, $R_{10}$ and $R_{11}$, are needed to store the results of $N_1,...,N_5$.
The importance of minimizing MF will be discussed in more detail in Section~\ref{sec:mot}.
Given an execution sequence of the netlist, we can easily obtain the corresponding minimum MF by deleting the operation results from the memory once they are not needed any more and storing the result of the scheduled operation at each clock cycle in the available row with the smallest index.
Different execution sequences have different minimum MF.
For example, if we swap the execution order of $N_3$ and $N_4$ in Fig.~\ref{fig:compiler}(c), the minimum MF becomes three.
Hence, the target of scheduler is to find the execution sequence with less corresponding minimum MF.

\subsection{Resubstitution}\label{sec:back_resub}

Resubstitution is a powerful method in logic synthesis aiming at reducing the size of a netlist~\cite{SIMRESUB}.
Its main idea is to check whether the function of a node, called \emph{root node}, in the netlist can be expressed using other existing nodes, called \emph{divisors}.
If so, we substitute the root node with the expression we find, and all nodes that are used exclusively by the root node, \textit{i.e.}, its \emph{maximum fanout free cone (MFFC)}~\cite{WINDRESUB}, can be deleted, thus reducing the size of the netlist.

A state-of-the-art resubstitution method is the simulation-guided resubstitution~\cite{SIMRESUB}.
It first simulates the netlist with some selected input patterns and stores the simulation results.
Then it traverses the netlist, treating each node as the root node, and collects a subset of the nodes in the netlists as its potential divisors.
Next, the algorithm checks for the existence of an expression with the simulation results.
The expression is usually either a divisor itself or a supported operation with the divisors as its inputs.
For example, in XMG, we check whether $r=d_1$, $r=\textit{XOR}(d_1,d_2,d_3)$, and $r=\textit{MAJ}(d_1,d_2,d_3)$, where $r$ is the root node, and $d_1,d_2,d_3$ are the possibly complemented divisors.
When such an expression exists, its function still may differ from that of the root node since there are input patterns not used in the simulation.
We call the expression found in this way a \emph{candidate}, and a satisfiability (SAT) validator is used to check whether a candidate is really functionally equivalent to the root node.
The candidate is used to substitute the root node only if it passes the equivalence checking.
% The process can be further improved by using don't cares and a normalization technique~\cite{SIMRESUB}.

==> 3_related.tex <==
\section{Related Works and Motivation}\label{sec:related}
In this section, we introduce some existing compilers for SIMD IMC and our motivation for an efficient compiler.
\subsection{Related Works}
Most existing compilers are based on the basic compiling flow to obtain one design of the target function.
Some works focus on improving the scheduling process of the compiler~\cite{SIMPLER,STAR,LOGIC,PREV}.
They use logic synthesis tools such as ABC~\cite{ABC} and Mockturtle~\cite{EPFLLIB} to perform the logic synthesis and apply some optimization commands in the tool to reduce the size of the netlist. 
For scheduling, they propose heuristic~\cite{SIMPLER,STAR,LOGIC} and divide-and-conquer~\cite{PREV} methods to obtain an execution sequence of the operations.
The performance is mainly evaluated in terms of the MF~\cite{SIMPLER,STAR,LOGIC,PREV}, other hardware-specific metrics such as the number of erasing cycles~\cite{STAR}, and throughput comparing to non-SIMD design style~\cite{SIMPLER,STAR}.
In~\cite{LOGIC}, an extra data layout reorganization algorithm is proposed to further improve the performance of sparse matrix-vector multiplication.
In~\cite{MIG}, the authors modify the Majority-Inverter Graph (MIG) optimization algorithm so that the operations with multiple complemented edges are reduced, since performing those operations require extra clock cycles and rows on the target device~\cite{PLIM}.
They also propose their own scheduling algorithm, and the experimental result is presented in terms of the number of operations, the number of clock cycles and MF.
These compilers are convenient to implement and relatively fast, but can only produce one design whose performance may be sub-optimal, since the final quality of a synthesized netlist cannot be predicted before scheduling.

In a recent work~\cite{XMG-GPPIC}, the authors explore over different netlist representations of the same function with an RL-framework to find the one with best end-to-end performance.
They start from the naive design synthesized by Mockturtle~\cite{EPFLLIB} and scheduled with the scheduler in~\cite{MIG}, and tempt to find a sequence of optimization commands so that after applying it to the naive netlist, the resulting netlist has good performance after scheduling.
The state space consists of netlist topology and some historical data, the action space consists of several optimization commands in Mockturtle~\cite{EPFLLIB}, and the reward is the improvement of performance in terms of energy or delay.
The experimental result shows that the EDP of the design obtained by RL-framework is greatly reduced compared to that of the naive design.
However, due to the long run time of RL algorithm, the optimization command sequence only contains 10 element.
Also, the scheduler used in the compiler is very simple, so the result may still be unsatisfactory.

\subsection{Motivation}
In all of these previous works, the synthesis and scheduling processes are decoupled.
Since it is hard to identify the characteristic of an un-scheduled netlist that makes the resulting design of good performance, the decoupled process greatly limits the quality of the design obtained.
Hence, we want to build a compiler with tight coupling of synthesis and scheduling.
Also, the performance of scheduler has a great impact on that of the compiler, so we use the state-of-the-art scheduler proposed in~\cite{PREV}.
Although~\cite{PREV} can achieve less MF than heuristic schedulers, its runtime is much larger due to the use of integer linear programming (ILP) and satisfiability modulo theories (SMT) solvers.
Hence, the compiler flows such as the RL-based one in~\cite{XMG-GPPIC} that requires to obtain scheduling result of many netlists are not applicable.
Therefore, an efficient compiler that can find high quality designs by exploring small amount of netlists is needed.
